CNN-Cert: An Efficient Framework for Certifying Robustness of Convolutional Neural Networks

Verifying robustness of neural network classifiers has attracted great interests and attention due to the success of deep neural networks and their unexpected vulnerability to adversarial perturbations. Although finding minimum adversarial distortion of neural networks (with ReLU activations) has been shown to be an NP-complete problem, obtaining a non-trivial lower bound of minimum distortion as a provable robustness guarantee is possible. However, most previous works only focused on simple fully-connected layers (multilayer perceptrons) and were limited to ReLU activations. This motivates us to propose a general and efficient framework, CNN-Cert, that is capable of certifying robustness on general convolutional neural networks. Our framework is general -- we can handle various architectures including convolutional layers, max-pooling layers, batch normalization layer, residual blocks, as well as general activation functions; our approach is efficient -- by exploiting the special structure of convolutional layers, we achieve up to 17 and 11 times of speed-up compared to the state-of-the-art certification algorithms (e.g. Fast-Lin, CROWN) and 366 times of speed-up compared to the dual-LP approach while our algorithm obtains similar or even better verification bounds. In addition, CNN-Cert generalizes state-of-the-art algorithms e.g. Fast-Lin and CROWN. We demonstrate by extensive experiments that our method outperforms state-of-the-art lower-bound-based certification algorithms in terms of both bound quality and speed.

==> _Tabfull_pureconv.tex <==

%%% the full simulations results 
%% part of the results are shown in the main paper


\begin{table*}[t]
\centering
\caption{Additional results: Averaged bounds on \textbf{(I) pure CNN networks with ReLU activations}}
\begin{adjustbox}{max width=0.93\textwidth}
\begin{tabular}{c|ccccc|cc|c}
\hline
Network & \multicolumn{5}{c|}{Certified Bounds} & \multicolumn{2}{c|}{\cnncertada Improvement (\%)} & Attack \\
\hline
      & $\ell_p$ norm & \cnncertada & \fastlin & Global-Lips & Dual-LP & vs. Fast-Lin & vs. Dual-LP & CW/EAD \\
\hline
MNIST, 2 layer & $\ell_\infty$ & 0.0416 & 0.0363 & 0.0071 & -     & +15\% & -     & - \\
5 filters & $\ell_2$ & 0.1572 & 0.1384 & 0.2574 & -     & +14\% & -     & - \\
3380 hidden nodes & $\ell_1$ & 0.3266 & 0.2884 & 0.9868 & -     & +13\% & -     & - \\
\hline
MNIST, 3 layer & $\ell_\infty$ & 0.0426 & 0.0381 & 0.0017 & -     & +12\% & -     & - \\
5 filters & $\ell_2$ & 0.2225 & 0.1925 & 0.1219 & -     & +16\% & -     & - \\
6260 hidden nodes & $\ell_1$ & 0.5061 & 0.4372 & 0.1698 & -     & +16\% & -     & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 0.0492 & 0.0406 & 0.0002 & 0.0456 & +21\% & +8\%  & 0.1488 \\
5 filters & $\ell_2$ & 0.1794 & 0.1453 & 0.0491 & 0.1653 & +23\% & +9\%  & 3.1407 \\
8680 hidden nodes & $\ell_1$ & 0.3363 & 0.2764 & 0.0269 & 0.3121 & +22\% & +8\%  & 14.4516 \\
\hline
MNIST, 5 layer & $\ell_\infty$ & 0.0306 & 0.0248 & 0.0000 & -     & +23\% & -     & - \\
5 filters & $\ell_2$ & 0.1263 & 0.1007 & 0.0235 & -     & +25\% & -     & - \\
10680 hidden nodes & $\ell_1$ & 0.2482 & 0.2013 & 0.0049 & -     & +23\% & -     & - \\
\hline
MNIST, 6 layer & $\ell_\infty$ & 0.0244 & 0.0195 & 0.0000 & -     & +25\% & -     & - \\
5 filters & $\ell_2$ & 0.0823 & 0.0664 & 0.0102 & -     & +24\% & -     & - \\
12300 hidden nodes & $\ell_1$ & 0.1517 & 0.1217 & 0.0006 & -     & +25\% & -     & - \\
\hline
MNIST, 7 layer & $\ell_\infty$ & 0.0267 & 0.0228 & 0.0000 & -     & +17\% & -     & - \\
5 filters & $\ell_2$ & 0.1046 & 0.0872 & 0.0033 & -     & +20\% & -     & - \\
13580 hidden nodes & $\ell_1$ & 0.1913 & 0.1578 & 0.0001 & -     & +21\% & -     & - \\
\hline
MNIST, 8 layer & $\ell_\infty$ & 0.0237 & 0.0203 & 0.0000 & -     & +17\% & -     & 0.1641 \\
5 filters & $\ell_2$ & 0.0877 & 0.0734 & 0.0017 & -     & +19\% & -     & 3.0014 \\
14560 hidden nodes & $\ell_1$ & 0.1540 & 0.1284 & 0.0000 & -     & +20\% & -     & 11.3418 \\
\hline
CIFAR, 5 layer & $\ell_\infty$ & 0.0070 & 0.0063 & 0.0000 & -     & +11\% & -     & 0.0241 \\
5 filters & $\ell_2$ & 0.0574 & 0.0494 & 0.0168 & -     & +16\% & -     & 0.5903 \\
14680 hidden nodes & $\ell_1$ & 0.1578 & 0.1348 & 0.0037 & -     & +17\% & -     & 15.6084 \\
\hline
CIFAR, 6 layer & $\ell_\infty$ & 0.0035 & 0.0031 & 0.0000 & -     & +13\% & -     & - \\
5 filters & $\ell_2$ & 0.0274 & 0.0231 & 0.0021 & -     & +19\% & -     & - \\
17100 hidden nodes & $\ell_1$ & 0.0775 & 0.0649 & 0.0001 & -     & +19\% & -     & - \\
\hline
CIFAR, 7 layer & $\ell_\infty$ & 0.0042 & 0.0036 & 0.0000 & -     & +17\% &  -    & 0.0229 \\
5 filters & $\ell_2$ & 0.0340 & 0.0287 & 0.0023 & -     & +18\% &  -    & 0.6612 \\
19100 hidden nodes & $\ell_1$ & 0.1009 & 0.0843 & 0.0001 & -     & +20\% &  -    & 12.5444 \\
\hline
CIFAR, 8 layer & $\ell_\infty$ & 0.0029 & 0.0026 & 0.0000 & -     & +12\% & -     & - \\
5 filters & $\ell_2$ & 0.0270 & 0.0228 & 0.0008 & -     & +18\% & -     & - \\
20720 hidden nodes & $\ell_1$ & 0.0834 & 0.0698 & 0.0000 & -     & +19\% & -     & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 0.0355 & 0.0310 & 0.0001 & -     & +15\% & -     & - \\
10 filters & $\ell_2$ & 0.1586 & 0.1336 & 0.0422 & -     & +19\% & -     & - \\
17360 hidden nodes & $\ell_1$ & 0.3360 & 0.2818 & 0.0130 & -     & +19\% & -     & - \\
\hline
MNIST, 8 layer & $\ell_\infty$ & 0.0218 & 0.0180 & 0.0000 & -     & +21\% & -     & - \\
10 filters & $\ell_2$ & 0.0884 & 0.0714 & 0.0006 & -     & +24\% & -     & - \\
29120 hidden nodes & $\ell_1$ & 0.1734 & 0.1394 & 0.0000 & -     & +24\% & -     & - \\
\hline
CIFAR, 5 layer & $\ell_\infty$ & 0.0042 & 0.0037 & 0.0000 & -     & +14\% & -     & - \\
10 filters & $\ell_2$ & 0.0324 & 0.0277 & 0.0042 & -     & +17\% & -     & - \\
29360 hidden nodes & $\ell_1$ & 0.0953 & 0.0806 & 0.0005 & -     & +18\% & -     & - \\
\hline
CIFAR, 7 layer & $\ell_\infty$ & 0.0030 & 0.0026 & 0.0000 & -     & +15\% & -     & - \\
10 filters & $\ell_2$ & 0.0228 & 0.0189 & 0.0005 & -     & +21\% & -     & - \\
38200 hidden nodes & $\ell_1$ & 0.0635 & 0.0521 & 0.0000 & -     & +22\% & -     & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 0.0341 & 0.0291 & 0.0000 & -     & +17\% & -     & - \\
20 filters & $\ell_2$ & 0.1243 & 0.1039 & 0.0221 & -     & +20\% & -     & - \\
34720 hidden nodes & $\ell_1$ & 0.2404 & 0.1993 & 0.0032 & -     & +21\% & -     & - \\
\hline
\end{tabular}%
\end{adjustbox}
\label{tab:addlabel}%

\end{table*}
\begin{table*}



\centering
\caption{Runtimes to find bounds of minimum adversarial distortion on pure CNN networks}
\begin{adjustbox}{max width=0.93\textwidth}
\begin{tabular}{c|ccccc|ccc}
\hline
Network & \multicolumn{5}{c|}{Average Computation Time (sec)} & \multicolumn{3}{c}{\cnncertada Speed-up} \\
\hline
      & $\ell_p$ norm & \cnncertada & \fastlin & Global-Lips & Dual-LP & vs. Fast-Lin, sparse & vs. Fast-Lin & vs. Dual-LP \\
\hline
MNIST, 2 layer & $\ell_\infty$ & 0.06  & 0.78  & 0.0001 & -     & 25.2  & 12.7  & - \\
5 filters & $\ell_2$ & 0.06  & 0.71  & 0.0002 & -     & 20.9  & 11.7  & - \\
3380 hidden nodes & $\ell_1$ & 0.05  & 0.74  & 0.0001 & -     & 25.1  & 14.2  & - \\
\hline
MNIST, 3 layer & $\ell_\infty$ & 0.25  & 4.02  & 0.0001 & -     & 9.4   & 15.9  & - \\
5 filters & $\ell_2$ & 0.25  & 3.99  & 0.0001 & -     & 9.2   & 15.8  & - \\
6260 hidden nodes & $\ell_1$ & 0.26  & 4.43  & 0.0001 & -     & 9.6   & 17.2  & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 0.91  & 12.11 & 0.0001 & 853.20 & 5.2   & 13.3  & 70.5 \\
5 filters & $\ell_2$ & 0.98  & 12.20 & 0.0001 & 236.30 & 5.0   & 12.5  & 19.4 \\
8680 hidden nodes & $\ell_1$ & 0.92  & 12.02 & 0.0001 & 227.69 & 5.1   & 13.0  & 18.9 \\
\hline
MNIST, 5 layer & $\ell_\infty$ & 2.41  & 16.85 & 0.0001 & -     & 3.0   & 7.0   & - \\
5 filters & $\ell_2$ & 2.25  & 17.11 & 0.0001 & -     & 3.0   & 7.6   & - \\
10680 hidden nodes & $\ell_1$ & 2.31  & 17.20 & 0.0001 & -     & 3.0   & 7.5   & - \\
\hline
MNIST, 6 layer & $\ell_\infty$ & 4.71  & 25.91 & 0.0001 & -     & 2.1   & 5.5   & - \\
5 filters & $\ell_2$ & 4.68  & 26.18 & 0.0002 & -     & 2.3   & 5.6   & - \\
12300 hidden nodes & $\ell_1$ & 4.64  & 25.94 & 0.0001 & -     & 2.2   & 5.6   & - \\
\hline
MNIST, 7 layer & $\ell_\infty$ & 8.23  & 32.38 & 0.0001 & -     & 1.5   & 3.9   & - \\
5 filters & $\ell_2$ & 8.24  & 33.36 & 0.0002 & -     & 1.6   & 4.0   & - \\
13580 hidden nodes & $\ell_1$ & 8.20  & 34.98 & 0.0001 & -     & 1.6   & 4.3   & - \\
\hline
MNIST, 8 layer & $\ell_\infty$ & 13.67 & 45.92 & 0.0001 & -     & 1.2   & 3.4   & - \\
5 filters & $\ell_2$ & 14.14 & 47.44 & 0.0002 & -     & 1.2   & 3.4   & - \\
14560 hidden nodes & $\ell_1$ & 12.82 & 112.29 & 0.0009 & -     & 1.6   & 8.8   & - \\
\hline
CIFAR, 5 layer & $\ell_\infty$ & 8.06  & 98.65 & 0.0001 & -     & 3.6   & 12.2  & - \\
5 filters & $\ell_2$ & 4.18  & 42.16 & 0.0001 & -     & 2.8   & 10.1  & - \\
14680 hidden nodes & $\ell_1$ & 4.17  & 39.65 & 0.0001 & -     & 2.9   & 9.5   & - \\
\hline
CIFAR, 6 layer & $\ell_\infty$ & 8.49  & 56.91 & 0.0001 & -     & 2.0   & 6.7   & - \\
5 filters & $\ell_2$ & 8.51  & 52.42 & 0.0001 & -     & 1.9   & 6.2   & - \\
17100 hidden nodes & $\ell_1$ & 8.41  & 55.18 & 0.0001 & -     & 2.0   & 6.6   & - \\
\hline
CIFAR, 7 layer & $\ell_\infty$ & 15.11 & 78.04 & 0.0001 & -     & 1.5   & 5.2   & - \\
5 filters & $\ell_2$ & 16.11 & 73.08 & 0.0001 & -     & 1.4   & 4.5   & - \\
19100 hidden nodes & $\ell_1$ & 14.93 & 76.89 & 0.0001 & -     & 1.5   & 5.1   & - \\
\hline
CIFAR, 8 layer & $\ell_\infty$ & 23.63 & 89.88 & 0.0001 & -     & 1.3   & 3.8   & - \\
5 filters & $\ell_2$ & 28.87 & 121.58 & 0.0001 & -     & 1.0   & 4.2   & - \\
20720 hidden nodes & $\ell_1$ & 23.63 & 121.44 & 0.0001 & -     & 1.2   & 5.1   & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 3.17  & -     & 0.0001 & -     & 3.6   & -     & - \\
10 filters & $\ell_2$ & 3.20  & -     & 0.0002 & -     & 3.5   & -     & - \\
17360 hidden nodes & $\ell_1$ & 3.16  & -     & 0.0001 & -     & 3.6   & -     & - \\
\hline
MNIST, 8 layer & $\ell_\infty$ & 61.74 & -     & 0.0001 & -     & 0.9   & -     & - \\
10 filters & $\ell_2$ & 61.72 & -     & 0.0001 & -     & 1.0   & -     & - \\
29120 hidden nodes & $\ell_1$ & 61.38 & -     & 0.0001 & -     & 0.9   & -     & - \\
\hline
CIFAR, 5 layer & $\ell_\infty$ & 17.18 & -     & 0.0001 & -     & 1.9   & -     & - \\
10 filters & $\ell_2$ & 17.11 & -     & 0.0001 & -     & 2.0   & -     & - \\
29360 hidden nodes & $\ell_1$ & 16.99 & -     & 0.0001 & -     & 1.9   & -     & - \\
\hline
CIFAR, 7 layer & $\ell_\infty$ & 67.23 & -     & 0.0001 & -     & 1.1   & -     & - \\
10 filters & $\ell_2$ & 67.13 & -     & 0.0001 & -     & 1.0   & -     & - \\
38200 hidden nodes & $\ell_1$ & 68.66 & -     & 0.0001 & -     & 1.1   & -     & - \\
\hline
MNIST, 4 layer & $\ell_\infty$ & 17.32 & -     & 0.0001 & -     & 2.0   & -     & - \\
20 filters & $\ell_2$ & 17.17 & -     & 0.0002 & -     & 2.1   & -     & - \\
34720 hidden nodes & $\ell_1$ & 17.23 & -     & 0.0001 & -     & 2.1   & -     & - \\
\hline
\end{tabular}%
\end{adjustbox}
\label{tab:addlabel}%



\end{table*}

==> definitions.tex <==
\newcommand{\hh}{H} % \nabla^2 \L(theta) 
\newcommand{\ggrad}{G} % \nabla   \L(theta) 

\def\covtype{{\sf covtype}\xspace}
\def\liblinear{{\sf LIBLINEAR}\xspace }
\def\LIBSVM{{\sf LIBSVM}\xspace}
\def\SVMLIGHT{{\sf SVMlight}\xspace}
\def\MNIST{{\sf mnist8m}\xspace}
\def\cifar{{\sf cifar}\xspace}
\def\ijcnn{{\sf ijcnn1}\xspace}
\def\covtype{{\sf covtype}\xspace}
\def\webspam{{\sf webspam}\xspace}

\newcommand{\lpfull}{{\small \textsf{LP-Full}}\xspace}
\newcommand{\reluplex}{{\small \textsf{Reluplex}}\xspace}
\newcommand{\crownada}{{\small \textsf{CROWN-Ada}}\xspace}
\newcommand{\crownquad}{{\small \textsf{CROWN-Quad}}\xspace}
\newcommand{\crown}{{\small \textsf{CROWN-general}}\xspace}
\newcommand{\crownName}{{\small \textsf{CROWN}}\xspace}
\newcommand{\fastlin}{{\small \textsf{Fast-Lin}}\xspace}
\newcommand{\fastlip}{{\small \textsf{Fast-Lip}}\xspace}


\def\bzero{{\boldsymbol 0}} 
\def\kappabar{\bar{\kappa}}
\def\psibar{\bar{\psi}}
\def\bdhat{\hat{{\boldsymbol d}}} 
\def\bdbar{\bar{{\boldsymbol d}}}
\def\underalpha{\underline{{\boldsymbol \alpha}} }
\def\fhatx{{\hat{f}_{\bx}}}
\def\fhatxH{{\hat{f}_{\bx, H}}}
\def\fhat{{\hat{f}}}
\def\bxp{{\boldsymbol x}_{+}}
\def\bxb{\bar{{\boldsymbol x}}}


\definecolor{LightCyan}{rgb}{0.88,1,1}
\def\sumbtheta{\bar{\btheta}}
\def\BigQUIC{{\sc BigQUIC}\xspace}
\def\PQN{{\sc PQN}~}
\def\Quad{{\sc QUIC}~}
\def\ALM{{\sc ALM}~}
\def\glasso{{\sc Glasso}~}
\def\IPM{{\sc IPM}~}
\def\PSM{{\sc PSM}~}
\def\CGD{{\sc CGD}~}
\def\sinco{{\sc SINCO}~}

\def\va{\mathbf{a}}
\def\vb{\mathbf{b}}
\def\vg{\mathbf{g}}
\def\vp{\mathbf{p}}
\def\vr{\mathbf{r}}
\def\vs{\mathbf{s}}
\def\vv{\mathbf{v}}
\def\vu{\mathbf{u}}
\def\vw{\mathbf{w}}
\def\vx{\mathbf{x}}
\def\vy{\mathbf{y}}
\def\vz{\mathbf{z}}
\def\ve{\mathbf{e}}
%\def\A{\mathcal{A}}

\newcommand{\cS}{\mathcal{S}}
\def\Leu{{\sf Leukemia}\xspace}
\def\ER{{\sf ER}\xspace}
\def\Climate{{\sf Climate}\xspace}
\def\Stock{{\sf Stock}\xspace}
\def\Synthetic{{\sf Synthetic}\xspace}
\def\bdelta{{\boldsymbol \Delta}}
\def\brho{{\boldsymbol \rho}}
\def\btheta{{\boldsymbol \theta}}
\def\Srfixed{{\mathcal{S}^{(r)}_\text{fixed}}}
\def\Srfree{{\mathcal{S}^{(r)}_\text{free}}}
\def\Sfree{{\mathcal{S}_\text{free}}}
\def\Sfixed{{\mathcal{S}_\text{fixed}}}


\def\bw{{\boldsymbol w}}
\newcommand{\V}{{\mathcal{V}}}
\def\N{\mathcal{N}}
\newcommand{\sign}{\operatorname{sign}}
\def\Soft{\mathcal{S}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\tr}{\operatorname{tr}}
\def\DeltaX{{\Delta}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\rl}[2]{\mathbb{R}^{{#1} \times {#2}}}
\newcommand{\half}{\frac{1}{2}}
\renewcommand{\vec}[1]{\bm{{#1}}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\proj}{\textsf{P}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\abs}[1]{\left\vert {#1} \right\vert}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\dom}{dom}
\renewcommand{\phi}{\varphi}
\newcommand{\coll}[1]{{\cal #1}}
\newcommand{\vct}[1]{\bm{#1}}

\def\bp{{\boldsymbol p}} 
\def\bg{{\boldsymbol g}}
\def\bs{{\boldsymbol s}}
\def\by{{\boldsymbol y}}
\def\bz{{\boldsymbol z}}
\def\bd{{\boldsymbol d}}
\def\bb{{\boldsymbol b}}
\def\bw{{\boldsymbol w}}
\def\bx{{\boldsymbol x}}
\def\bv{{\boldsymbol v}}
\def\bu{{\boldsymbol u}}
\def\ba{{\boldsymbol a}}
\def\be{{\boldsymbol e}}
\def\br{{\boldsymbol r}}
\def\AL{{\boldsymbol \alpha}}
%\def\W{\mathcal{W}}
\def\G{\mathcal{G}}
\def\T{\mathcal{T}}
\def\J{\mathcal{J}}
\def\D{\mathcal{D}}
\def\S{\mathcal{S}}
\def\C{\mathcal{C}}
%\def\A{\mathcal{A}}
\def\RR{\mathbb{R}}
\def\S{\mathcal{S}}
\def\N{\mathcal{N}}
\def\L{\mathcal{L}}
\DeclareMathOperator{\prox}{prox}

\newcommand{\Rspace}[1]{\mathbb{R}^{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\ip}[2]{\langle {#1}, {#2} \rangle}
\newcommand{\dotproduct}[2]{#1^T #2}
\newcommand{\diag}[1]{\operatorname{diag}{#1}} 
\newcommand{\trace}[1]{\operatorname{trace}({#1})}
\newcommand{\grad}{\nabla}
\newcommand{\breg}[2]{D_\varphi({#1};\ {#2})}
\newcommand{\realsplus}[1]{\reals_+^{#1}}
\renewcommand{\vec}[1]{\bm{ {#1} }}
\newcommand{\frob}[1]{\| {#1} \|_{\text{F}}}
\newcommand{\Sig}{\bm{\Sigma}}

%\usepackage[pdftex]{graphicx}
%\usepackage{sidecap}
\def\pitem{\item}
